Library Liberation: Competitive Performance Matmul Through Compiler-composed Nanokernels

The rapidly evolving landscape of AI and machine learning workloads has widened the gap between high-level domain operations and efficient hardware utilization. Achieving near-peak performance still demands deep hardware expertise-experts either handcraft target-specific kernels (e.g., DeepSeek) or rely on specialized libraries (e.g., CUTLASS)-both of which add complexity and limit scalability for most ML practitioners. This paper introduces a compilation scheme that automatically generates scalable, high-performance microkernels by leveraging the MLIR dialects to bridge domain-level operations and processor capabilities. Our approach removes dependence on low-level libraries by enabling the compiler to auto-generate near-optimal code directly. At its core is a mechanism for composing nanokernels from low-level IR constructs with near-optimal register utilization, forming efficient microkernels tailored to each target. We implement this technique in an MLIR-based compiler supporting both vector and tile based CPU instructions. Experiments show that the generated nanokernels are of production-quality, and competitive with state-of-the-art microkernel libraries.

==> 02_motivation.tex <==
ML workloads are fundamentally built upon two computational primitives: contractions and elementwise operations~\cite{mlperf-infer, mlperf-train, fathom}. Although contractions can achieve high computational intensity and approach peak performance when executed in isolation, the reality of neural network execution reveals a critical performance bottleneck: the memory wall between operations.
This limitation is commonly addressed by operation fusion~\cite{dl-comp-survey, onednn, flashattention} which optimizes memory access traffic.

Automatic optimizations have long been the key goal of modern compilers. Code simplification and reuse, strength reduction, data access optimizations are steps that modern compilers perform well~\cite{llvmir, tvm}. However, strong loop vectorization, the key to accelerating compute-dense operations such as General Matrix Multiply (GEMM), has eluded automation using purely mathematical approaches such as polyhedral analysis~\cite{polyhedral}.
As an alternative, many domain-specific languages (DSLs)~\cite{triton, tensorcomprehensions} and optimized libraries~\cite{libxsmm, pytorch} have been created. These specific solutions often lag in the adoption of new hardware features and lack support for novel operations~\cite{flashattention3, fast-alg-cnn}. 

A growing need for scalable and automated support for the fusion of ML operations remains. The increasing complexity of managing these individual solutions has led to the creation of additional abstractions (TPP, MLIR~\cite{mlir}) to reduce that complexity.
We start by focusing on enabling high-performance code generation by embedding expert library-writer knowledge directly into a compiler for the key ML operation: contraction. Creating a robust and reusable compilation infrastructure can ensure a sustainable platform for further optimizations.


% AI workloads are fundamentally built upon two computational primitives: General Matrix Multiply (GEMM) operations and elementwise operations. While GEMM operations can achieve high computational intensity and approach peak performance when executed in isolation, the reality of neural network execution reveals a critical performance bottleneck: the memory wall between operations.
% AI workloads face acute memory wall challenges through cascading operation sequences like ReLU(BatchNorm(GEMM(input))). When compiled independently, each operation forces expensive memory round-trips, generating multiple times the necessary memory traffic and transforming compute-intensive workloads into memory-bound operations that underutilize available processing capacity.
% Achieving peak performance requires orchestrating complex optimizations involving vector register management, operation fusion, and thereby optimizing memory access traffic.
% Automatic optimization has long been a key goal of modern compilers. Code simplification and reuse,  strength reduction, data access optimizations are steps that most modern compilers perform well.
% For high-performance problems, most of the time and effort is spent inside tight loops performing repetitive tasks, but strong loop vectorization has eluded purely mathematical approaches such as polyhedral analysis~\cite{polyhedral}.
% To fill this gap, countless \textit{optimized libraries} have been produced over the years on various levels of programmability.

% Optimized libraries are hard to use in general code, so an equal number of \textit{frameworks} and \textit{DSLs} have been created to help program with those libraries, or hide them completely from the programmer.
% However, this makes it harder to keep the whole compilation process simple, so various levels of abstractions (TPP, MLIR~\cite{mlir}, LLVM IR~\cite{llvmir}) have converged to reduce that complexity.

% Micro-kernel libraries such as LIBXSMM and oneDNN~\cite{onednn} use similar abstractions at different levels, but both need support from a compiler or framework to dispatch the appropriate kernels for the right user code.
% To avoid the combinatorial explosion of a fat-binary, these libraries utilize a JIT-compiler approach that creates the micro-kernels on demand at run time, which creates another level of complexity and adds a new point of failure.
% In addition, even expertly crafted compilers (e.g. TPP-MLIR) have trouble making use of such vast number of possibilities and performance profiles of the JIT-compiler, especially considering that these two programs have different development cadence and external interferences (for example, an LLVM-based compiler that follows the upstream branch closely).



==> 08_future.tex <==
\subsection{Nanokernel generation for other architectures}
Athough we proposed our nanokernel techniques targeting mainly the {\tt x86} architecture, it could be generalized for other architectures like {\tt Aarch64} and {\tt RISC-V}. The FP32 nanokernel generation is $generic$ and could be used for any target architecture because it depends on  generalized {\tt vector} operations. For BF16 type, if the {\tt Aarch64} or {\tt RISC-V} architecture supports its own BF16 dot-product then a new lowering has to be defined for their vector and matrix extensions like we did for {\tt AMX} and {\tt DotBBF16Op}.

\subsection{Nanokernel generation for other packed types}
We can extend or follow  the BF16 nanokernel technique to support other packed types like Int8 and F16. For example, Intel's ArrowLake machine supports  {\tt avx.dot.i8} Int8 operation (like {\tt avx512.dot} BF16 operation) to perform dot product. We could follow the {\tt DotBF16Op} technique to load the A subrow and B subcolumn 
and perform {\tt avx.dot.i8} operation instead of {\tt avx512.dot}. Similalry, with the AVX2 Packed Instruction set we can load or broadcast F16 type elements to F32 and perform FMAs.
Currently, we are generalizing the BF16 nanokernel technique independent of target architecture and planning to upstream both FP32 and BF16 techniques into MLIR/LLVM compiler infrastructure. Afterwards, extend the nanokernel generation for Int8 type along with quantization support as a future work.



% \begin{tikzpicture}[every node/.style={font=\small}]

% % Original 4x4 matrix
% \matrix (m1) [matrix of nodes,
%               nodes in empty cells,
%               nodes={draw, minimum size=8mm, anchor=center}]
% {
%   1 & 2 & 3 & 4 \\
%   5 & 6 & 7 & 8 \\
%   9 & 10 & 11 & 12 \\
%   13 & 14 & 15 & 16 \\
% };
% %\node[above=3mm of m1-1-2] {Original 4x4 Matrix};

% % VNNI packed matrix, placed to the right
% \matrix (m2) [matrix of nodes,
%               nodes in empty cells,
%               nodes={draw, minimum size=15mm, anchor=center},
%               right=3cm of m1]
% {
%   (1,5) & (2,6) & (3,7) & (4,8) \\
%   (9,13) & (10,14) & (11,15) & (12,16) \\
% };
% %\node[above=3mm of m2-1-2] {VNNI Packed Matrix};

% % Arrow between them
% %\draw[->, thick] (m1.east) -- (m2.west) node[midway, above] {packing};

% \end{tikzpicture}

% \[
% \begin{bmatrix}
% a_{11} & a_{12} & a_{13} & a_{14} \\
% a_{21} & a_{22} & a_{23} & a_{24} \\
% a_{31} & a_{32} & a_{33} & a_{34} \\
% a_{41} & a_{42} & a_{43} & a_{44}
% \end{bmatrix}
% \]

% \[
% \begin{bmatrix}
% a_{11} & a_{12} & a_{13} & a_{14} \\
% a_{21} & a_{22} & a_{23} & a_{24} \\
% a_{31} & a_{32} & a_{33} & a_{34} \\
% a_{41} & a_{42} & a_{43} & a_{44}
% \end{bmatrix}
% \qquad
% \begin{bmatrix}
% b_{11} & b_{12} & b_{13} & b_{14} \\
% b_{21} & b_{22} & b_{23} & b_{24} \\
% b_{31} & b_{32} & b_{33} & b_{34} \\
% b_{41} & b_{42} & b_{43} & b_{44}
% \end{bmatrix}
% \]

% \begin{figure}[h!]
%     \centering
%     \begin{tikzpicture}
%         % First matrix
%         \matrix (A) [matrix of math nodes,left delimiter={[},right delimiter={]}] {
%             0 & 1 & 2 & 3 \\
%             4 & 5 & 6 & 7 \\
%             8 & 9 & 10 & 11 \\
%             12 & 13 & 14 & 15 \\
%         };
%         \node[below=5pt of A.south] {(a) Flat 4$\times$4 matrix};

%         % Second matrix
%         \matrix (B) [matrix of math nodes,right=0.5cm of A,right delimiter={]},left delimiter={[}] {
%             (0, 4) & (1, 5)  & (2,6) & (3,7) \\
%             (8, 12) & (9, 13)  & (10, 14) & (11, 15) \\
%         };
%         \node[below=14pt of B.south] {(b) VNNI packed 4$\times$2$\times$2 matrix};
%     \end{tikzpicture}
    
%     \caption{Packing a 4$\times$4 row-major order matrix to VNNI}
%     \label{fig:vnni-packing}
% \end{figure}
    



% \textcolor{red}{Quantization?
% GPU?
% MHA?}

==> fig/register-block-mn.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,149); %set diagram left start at 0, and has height of 149

%Shape: Grid [id:dp13729621992433816] 
\draw  [draw opacity=0][fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.35 ] (289.13,51.88) -- (350.73,51.88) -- (350.73,133.88) -- (289.13,133.88) -- cycle ; \draw   (289.13,51.88) -- (289.13,133.88)(309.13,51.88) -- (309.13,133.88)(329.13,51.88) -- (329.13,133.88)(349.13,51.88) -- (349.13,133.88) ; \draw   (289.13,51.88) -- (350.73,51.88)(289.13,71.88) -- (350.73,71.88)(289.13,91.88) -- (350.73,91.88)(289.13,111.88) -- (350.73,111.88)(289.13,131.88) -- (350.73,131.88) ; \draw    ;
%Shape: Grid [id:dp7554541297379229] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.25 ] (211.73,51.95) -- (233.13,51.95) -- (233.13,132.88) -- (211.73,132.88) -- cycle ; \draw   (211.73,51.95) -- (211.73,132.88)(231.73,51.95) -- (231.73,132.88) ; \draw   (211.73,51.95) -- (233.13,51.95)(211.73,71.95) -- (233.13,71.95)(211.73,91.95) -- (233.13,91.95)(211.73,111.95) -- (233.13,111.95)(211.73,131.95) -- (233.13,131.95) ; \draw    ;
%Shape: Grid [id:dp18863294368730965] 
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.25 ] (290.13,22.95) -- (351.73,22.95) -- (351.73,43.88) -- (290.13,43.88) -- cycle ; \draw   (290.13,22.95) -- (290.13,43.88)(310.13,22.95) -- (310.13,43.88)(330.13,22.95) -- (330.13,43.88)(350.13,22.95) -- (350.13,43.88) ; \draw   (290.13,22.95) -- (351.73,22.95)(290.13,42.95) -- (351.73,42.95) ; \draw    ;
%Shape: Grid [id:dp9402899229920767] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.4 ] (261.73,51.46) -- (283.13,51.46) -- (283.13,72.4) -- (261.73,72.4) -- cycle ; \draw   (261.73,51.46) -- (261.73,72.4)(281.73,51.46) -- (281.73,72.4) ; \draw   (261.73,51.46) -- (283.13,51.46)(261.73,71.46) -- (283.13,71.46) ; \draw    ;
%Straight Lines [id:da9413642739867143] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (230.47,61.4) -- (258.47,60.47) ;
\draw [shift={(260.47,60.4)}, rotate = 178.09] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2419806320837996] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (230.47,82.4) -- (258.85,61.58) ;
\draw [shift={(260.47,60.4)}, rotate = 143.75] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7947296456897275] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (230.47,100.4) -- (260.26,61) ;
\draw [shift={(261.47,59.4)}, rotate = 127.09] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2553809073070049] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (230.47,120.4) -- (261.55,60.18) ;
\draw [shift={(262.47,58.4)}, rotate = 117.3] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (295.13,24.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (315.13,24.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (336.13,24.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (293.13,52.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};
% Text Node
\draw (293.13,74.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {7};
% Text Node
\draw (290.13,93.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {10};
% Text Node
\draw (291.13,114.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {13};
% Text Node
\draw (313.13,53.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {5};
% Text Node
\draw (333.13,53.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {6};
% Text Node
\draw (314.13,74.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {8};
% Text Node
\draw (311.13,93.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {11};
% Text Node
\draw (311.13,114.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {14};
% Text Node
\draw (334.13,74.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {9};
% Text Node
\draw (331.13,94.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {12};
% Text Node
\draw (331.13,113.88) node [anchor=north west][inner sep=0.75pt]   [align=left] {15};
% Text Node
\draw (203.13,8.95) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {load chunk of Bi subcolumn in 3 vec registers};
% Text Node
\draw (197.98,138.24) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-269.44,xslant=0.04] [align=left] {broadcast Ai subrow};
% Text Node
\draw (358.98,136.24) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-269.44,xslant=0.04] [align=left] {Cj accumulator in\\12 vect register};
% Text Node
\draw (267.13,52.95) node [anchor=north west][inner sep=0.75pt]   [align=left] {0};


\end{tikzpicture}
